Enhancing Spatio-temporal Quantile Forecasting with Curriculum Learning: Lessons Learned

Training models on spatio-temporal (ST) data poses an open problem due to the complicated and diverse nature of the data itself, and it is challenging to ensure the model's performance directly trained on the original ST data. While limiting the variety of training data can make training easier, it can also lead to a lack of knowledge and information for the model, resulting in a decrease in performance. To address this challenge, we presented an innovative paradigm that incorporates three separate forms of curriculum learning specifically targeting from spatial, temporal, and quantile perspectives. Furthermore, our framework incorporates a stacking fusion module to combine diverse information from three types of curriculum learning, resulting in a strong and thorough learning process. We demonstrated the effectiveness of this framework with extensive empirical evaluations, highlighting its better performance in addressing complex ST challenges. We provided thorough ablation studies to investigate the effectiveness of our curriculum and to explain how it contributes to the improvement of learning efficiency on ST data.

==> table/old_exp.tex <==
\begin{table*}[h!]
\caption{Overall Comparison}
\label{main_experiment}
\tiny
\renewcommand{\arraystretch}{2}
\begin{tabular}{|l|llllllllllllllllll|}
\hline
& \multicolumn{6}{c|}{\textbf{Horizon 3}}   & \multicolumn{6}{c|}{\textbf{Horizon 6}}     & \multicolumn{6}{c|}{\textbf{Horizon 12}}   \\ \hline

\textbf{ \multirow{2}{*}{Models} }    & \multicolumn{1}{c|}{\textbf{RMSE}}     & \multicolumn{1}{c|}{\textbf{MAE}}      & \multicolumn{1}{c|}{\textbf{MAPE}}         & \multicolumn{1}{c|}{\textbf{Q10}}         & \multicolumn{1}{c|}{\textbf{Q50}}         & \multicolumn{1}{c|}{\textbf{Q90}}         & \multicolumn{1}{c|}{\textbf{RMSE}}         & \multicolumn{1}{c|}{\textbf{MAE}}          & \multicolumn{1}{c|}{\textbf{MAPE}}         & \multicolumn{1}{c|}{\textbf{Q10}}         & \multicolumn{1}{c|}{\textbf{Q50}}         & \multicolumn{1}{c|}{\textbf{Q90}}         & \multicolumn{1}{c|}{\textbf{RMSE}}         & \multicolumn{1}{c|}{\textbf{MAE}}          & \multicolumn{1}{c|}{\textbf{MAPE}}         & \multicolumn{1}{c|}{\textbf{Q10}}         & \multicolumn{1}{c|}{\textbf{Q50}}          & \multicolumn{1}{c|}{\textbf{Q90}} \\ \hline

\textbf{Datasets}        & \multicolumn{18}{c|}{\textbf{PEMS04}}                                                                                        \\ \hline

DeepAR & \multicolumn{1}{l|}{32.503}  & \multicolumn{1}{l|}{20.927}  & \multicolumn{1}{l|}{12.035}   & \multicolumn{1}{l|}{5.004}   & \multicolumn{1}{l|}{10.688}  & \multicolumn{1}{l|}{5.076} & \multicolumn{1}{l|}{36.441}  & \multicolumn{1}{l|}{23.154}   & \multicolumn{1}{l|}{13.313}  & \multicolumn{1}{l|}{5.942}     & \multicolumn{1}{l|}{12.064}   & \multicolumn{1}{l|}{6.245}  & \multicolumn{1}{l|}{41.958}      & \multicolumn{1}{l|}{26.665}   & \multicolumn{1}{l|}{15.384}   & \multicolumn{1}{l|}{6.753}         & \multicolumn{1}{l|}{12.668}    & 8.129    \\ \hline


MQRNN & \multicolumn{1}{l|}{30.794}                & \multicolumn{1}{l|}{19.279}                & \multicolumn{1}{l|}{11.332}                & \multicolumn{1}{l|}{4.521}                & \multicolumn{1}{l|}{9.763}                & \multicolumn{1}{l|}{4.581}                & \multicolumn{1}{l|}{33.983}                & \multicolumn{1}{l|}{21.631}                & \multicolumn{1}{l|}{12.655}                & \multicolumn{1}{l|}{5.073}                & \multicolumn{1}{l|}{10.816}               & \multicolumn{1}{l|}{5.018}                & \multicolumn{1}{l|}{39.256}                & \multicolumn{1}{l|}{25.412}                & \multicolumn{1}{l|}{15.217}                & \multicolumn{1}{l|}{6.089}                & \multicolumn{1}{l|}{12.706}                & 5.745                           \\ \hline


STGCN & \multicolumn{1}{l|}{30.522}                & \multicolumn{1}{l|}{19.167}                & \multicolumn{1}{l|}{11.350}                & \multicolumn{1}{l|}{4.552}                & \multicolumn{1}{l|}{9.702}                & \multicolumn{1}{l|}{4.418}                & \multicolumn{1}{l|}{32.305}                & \multicolumn{1}{l|}{20.234}                & \multicolumn{1}{l|}{11.914}                & \multicolumn{1}{l|}{4.829}                & \multicolumn{1}{l|}{10.243}               & \multicolumn{1}{l|}{4.707}                & \multicolumn{1}{l|}{35.098}                & \multicolumn{1}{l|}{22.192}                & \multicolumn{1}{l|}{13.113}                & \multicolumn{1}{l|}{5.318}                & \multicolumn{1}{l|}{11.229}                & 5.228                             \\ \hline

STGCN+QSTCL  & \multicolumn{1}{l|}{{\ul \textbf{29.884}}}                & \multicolumn{1}{l|}{{\ul \textbf{18.689}}}                & \multicolumn{1}{l|}{{\ul \textbf{11.022}}}                & \multicolumn{1}{l|}{{\ul \textbf{4.419}}}                & \multicolumn{1}{l|}{{\ul \textbf{9.463}}}               & \multicolumn{1}{l|}{{\ul \textbf{4.273}}}                & \multicolumn{1}{l|}{{\ul \textbf{31.567}}}                & \multicolumn{1}{l|}{{\ul \textbf{19.683}}}                & \multicolumn{1}{l|}{{\ul \textbf{11.529}}}                & \multicolumn{1}{l|}{{\ul \textbf{4.696}}}                & \multicolumn{1}{l|}{{\ul \textbf{9.967}}}               & \multicolumn{1}{l|}{{\ul \textbf{4.551}}}                & \multicolumn{1}{l|}{{\ul \textbf{34.177}}}                & \multicolumn{1}{l|}{{\ul \textbf{21.540}}}                & \multicolumn{1}{l|}{{\ul \textbf{12.586}}}                & \multicolumn{1}{l|}{{\ul \textbf{5.171}}}                & \multicolumn{1}{l|}{{\ul \textbf{10.906}}}                &    \multicolumn{1}{l|}{{\ul \textbf{5.039}}}                              \\ \hline


DCRNN & \multicolumn{1}{l|}{30.181}                & \multicolumn{1}{l|}{19.193}                & \multicolumn{1}{l|}{11.481}                & \multicolumn{1}{l|}{4.554}                & \multicolumn{1}{l|}{9.722}                & \multicolumn{1}{l|}{4.437}                & \multicolumn{1}{l|}{32.280}                & \multicolumn{1}{l|}{20.608}                & \multicolumn{1}{l|}{12.316}                & \multicolumn{1}{l|}{4.923}                & \multicolumn{1}{l|}{10.438}               & \multicolumn{1}{l|}{4.823}                & \multicolumn{1}{l|}{36.133}                & \multicolumn{1}{l|}{23.419}                & \multicolumn{1}{l|}{14.144}                & \multicolumn{1}{l|}{5.646}                & \multicolumn{1}{l|}{11.858}                & 5.639                           \\ \hline



DCRNN+QSTCL  & \multicolumn{1}{l|}{29.954}                & \multicolumn{1}{l|}{19.001}                & \multicolumn{1}{l|}{10.894}                & \multicolumn{1}{l|}{4.416}                & \multicolumn{1}{l|}{9.651}                & \multicolumn{1}{l|}{4.341}                & \multicolumn{1}{l|}{31.894}                & \multicolumn{1}{l|}{20.154}               & \multicolumn{1}{l|}{11.935}                & \multicolumn{1}{l|}{4.785}                & \multicolumn{1}{l|}{10.271}               & \multicolumn{1}{l|}{4.574}                & \multicolumn{1}{l|}{35.657}                & \multicolumn{1}{l|}{22.947}                & \multicolumn{1}{l|}{13.842}                & \multicolumn{1}{l|}{5.462}                & \multicolumn{1}{l|}{11.693}                & 5.484                          \\ \hline

GWN & \multicolumn{1}{l|}{29.237}                & \multicolumn{1}{l|}{18.050}                & \multicolumn{1}{l|}{10.805}                & \multicolumn{1}{l|}{4.313}                & \multicolumn{1}{l|}{9.14}                & \multicolumn{1}{l|}{4.105}                & \multicolumn{1}{l|}{30.852}                & \multicolumn{1}{l|}{19.020}                & \multicolumn{1}{l|}{11.366}                & \multicolumn{1}{l|}{4.621}                & \multicolumn{1}{l|}{9.634}               & \multicolumn{1}{l|}{4.378}                & \multicolumn{1}{l|}{33.124}                & \multicolumn{1}{l|}{20.579}                & \multicolumn{1}{l|}{12.325}                & \multicolumn{1}{l|}{5.059}                & \multicolumn{1}{l|}{10.416}                &   4.794                           \\ \hline


GWN+QSTCL  & \multicolumn{1}{l|}{{\ul \textbf{28.587}}}                & \multicolumn{1}{l|}{{\ul \textbf{17.625}}}                & \multicolumn{1}{l|}{{\ul \textbf{10.496}}}                & \multicolumn{1}{l|}{{\ul \textbf{4.186}}}                & \multicolumn{1}{l|}{{\ul \textbf{8.927}}}               & \multicolumn{1}{l|}{{\ul \textbf{4.002}}}                & \multicolumn{1}{l|}{{\ul \textbf{30.038}}}                & \multicolumn{1}{l|}{{\ul \textbf{18.490}}}                & \multicolumn{1}{l|}{{\ul \textbf{10.982}}}                & \multicolumn{1}{l|}{{\ul \textbf{4.458}}}                & \multicolumn{1}{l|}{{\ul \textbf{9.365}}}               & \multicolumn{1}{l|}{{\ul \textbf{4.248}}}                & \multicolumn{1}{l|}{{\ul \textbf{31.910}}}                & \multicolumn{1}{l|}{{\ul \textbf{19.820}}}                & \multicolumn{1}{l|}{{\ul \textbf{11.780}}}                & \multicolumn{1}{l|}{{\ul \textbf{4.812}}}                & \multicolumn{1}{l|}{{\ul \textbf{10.037}}}                &    \multicolumn{1}{l|}{{\ul \textbf{4.620}}}                              \\ \hline


STNorm & \multicolumn{1}{l|}{29.551}                & \multicolumn{1}{l|}{18.222}                & \multicolumn{1}{l|}{10.831}                & \multicolumn{1}{l|}{4.308}                & \multicolumn{1}{l|}{9.226}                & \multicolumn{1}{l|}{4.146}                & \multicolumn{1}{l|}{31.281}                & \multicolumn{1}{l|}{19.197}                & \multicolumn{1}{l|}{11.359}                & \multicolumn{1}{l|}{4.637}                & \multicolumn{1}{l|}{9.722}               & \multicolumn{1}{l|}{5.090}                & \multicolumn{1}{l|}{33.476}                & \multicolumn{1}{l|}{20.756}                & \multicolumn{1}{l|}{12.428}                & \multicolumn{1}{l|}{5.090}                & \multicolumn{1}{l|}{10.506}                &         4.825                 \\ \hline

STNorm-QSTCL & \multicolumn{1}{l|}{{\ul \textbf{29.263}}}                & \multicolumn{1}{l|}{{\ul \textbf{18.166} }}               & \multicolumn{1}{l|}{{\ul \textbf{10.806}  }}              & \multicolumn{1}{l|}{{\ul \textbf{4.258}}}                & \multicolumn{1}{l|}{{\ul \textbf{9.199}   }}             & \multicolumn{1}{l|}{{\ul \textbf{4.116}}}                & \multicolumn{1}{l|}{{\ul \textbf{30.867}}}                & \multicolumn{1}{l|}{{\ul \textbf{19.085}  }}              & \multicolumn{1}{l|}{{\ul \textbf{11.314} }}               & \multicolumn{1}{l|}{{\ul \textbf{4.550}}}                & \multicolumn{1}{l|}{{\ul \textbf{9.665}}}              & \multicolumn{1}{l|}{{\ul \textbf{4.365}}}                & \multicolumn{1}{l|}{{\ul \textbf{32.839}}}                & \multicolumn{1}{l|}{{\ul \textbf{20.395}}}                & \multicolumn{1}{l|}{{\ul \textbf{12.131}}}                & \multicolumn{1}{l|}{{\ul \textbf{4.939}}}                & \multicolumn{1}{l|}{{\ul \textbf{10.326}}}                &          {\ul \textbf{4.741}}                \\ \hline


SCINet & \multicolumn{1}{l|}{29.644}                & \multicolumn{1}{l|}{18.705}                & \multicolumn{1}{l|}{11.163}                & \multicolumn{1}{l|}{4.625}                & \multicolumn{1}{l|}{9.471}                & \multicolumn{1}{l|}{4.344}                & \multicolumn{1}{l|}{30.923}                & \multicolumn{1}{l|}{19.531}                & \multicolumn{1}{l|}{11.666}                & \multicolumn{1}{l|}{4.829}                & \multicolumn{1}{l|}{9.883}               & \multicolumn{1}{l|}{4.590 }                & \multicolumn{1}{l|}{33.605}                & \multicolumn{1}{l|}{21.550}                & \multicolumn{1}{l|}{13.024}                & \multicolumn{1}{l|}{5.295}                & \multicolumn{1}{l|}{10.899}                &          5.151                \\ \hline

SCINet-QSTCL & \multicolumn{1}{l|}{{\ul \textbf{29.571}}}                & \multicolumn{1}{l|}{{\ul \textbf{18.588}}}                & \multicolumn{1}{l|}{{\ul \textbf{11.042}}}                & \multicolumn{1}{l|}{{\ul \textbf{4.579}}}                & \multicolumn{1}{l|}{{\ul \textbf{9.408}}}                & \multicolumn{1}{l|}{{\ul \textbf{4.271}}}                & \multicolumn{1}{l|}{{\ul \textbf{30.871} }}               & \multicolumn{1}{l|}{{\ul \textbf{19.421}  }}              & \multicolumn{1}{l|}{{\ul \textbf{11.499}}}                & \multicolumn{1}{l|}{{\ul \textbf{4.807}}}                & \multicolumn{1}{l|}{{\ul \textbf{9.829}}}               & \multicolumn{1}{l|}{{\ul \textbf{4.511}  }}              & \multicolumn{1}{l|}{{\ul \textbf{33.371}}}                & \multicolumn{1}{l|}{{\ul \textbf{21.229}}}                & \multicolumn{1}{l|}{{\ul \textbf{12.618}}}                & \multicolumn{1}{l|}{{\ul \textbf{5.236}}}                & \multicolumn{1}{l|}{{\ul \textbf{10.741}}}                &          {\ul \textbf{4.999}}                \\ \hline


STAEFormer todo & \multicolumn{1}{l|}{29.292}                & \multicolumn{1}{l|}{17.589}                & \multicolumn{1}{l|}{11.993}                & \multicolumn{1}{l|}{4.190}                & \multicolumn{1}{l|}{8.794}                & \multicolumn{1}{l|}{3.921}                & \multicolumn{1}{l|}{30.931}                & \multicolumn{1}{l|}{18.371}                & \multicolumn{1}{l|}{12.435}                & \multicolumn{1}{l|}{4.486}                & \multicolumn{1}{l|}{9.186}               & \multicolumn{1}{l|}{4.141}                & \multicolumn{1}{l|}{32.922}                & \multicolumn{1}{l|}{19.543}                & \multicolumn{1}{l|}{13.171}                & \multicolumn{1}{l|}{4.844}                & \multicolumn{1}{l|}{9.772}                &          4.482                 \\ \hline

% | 3  Horizon | RMSE:  29.292; MAE:  17.589; MAPE: 11.993; Q10: 4.190; Q50: 8.794; Q90: 3.921;
% | 6  Horizon | RMSE:  30.931; MAE:  18.371; MAPE: 12.435; Q10: 4.486; Q50: 9.186; Q90: 4.141;
% | 12 Horizon | RMSE:  32.922; MAE:  19.543; MAPE: 13.171; Q10: 4.844; Q50: 9.772; Q90: 4.482;


STAEFormer-QSTCL  & \multicolumn{1}{l|}{{\ul \textbf{29.764}}}                & \multicolumn{1}{l|}{{\ul \textbf{17.718}}}                & \multicolumn{1}{l|}{{\ul \textbf{10.494}}}               & \multicolumn{1}{l|}{{\ul \textbf{4.381}}}                & \multicolumn{1}{l|}{{\ul \textbf{8.978}}}                & \multicolumn{1}{l|}{{\ul \textbf{4.101}}}                & \multicolumn{1}{l|}{{\ul \textbf{31.449}}}                & \multicolumn{1}{l|}{{\ul \textbf{18.534}}}                & \multicolumn{1}{l|}{{\ul \textbf{10.889}}}                & \multicolumn{1}{l|}{{\ul \textbf{4.702}}}                & \multicolumn{1}{l|}{{\ul \textbf{9.392}}}               & \multicolumn{1}{l|}{{\ul \textbf{4.387}}}                & \multicolumn{1}{l|}{{\ul \textbf{32.973}}}                & \multicolumn{1}{l|}{{\ul \textbf{19.528}}}                & \multicolumn{1}{l|}{{\ul \textbf{11.421}}}                & \multicolumn{1}{l|}{{\ul \textbf{4.959}}}                & \multicolumn{1}{l|}{{\ul \textbf{9.895}}}                &          {\ul \textbf{4.700}}                 \\ \hline


\textbf{Datasets}        & \multicolumn{18}{c|}{\textbf{METR-LA}}                                                                                        \\ \hline


DeepAR & \multicolumn{1}{l|}{7.357}  & \multicolumn{1}{l|}{3.373}  & \multicolumn{1}{l|}{8.213}   & \multicolumn{1}{l|}{1.142}   & \multicolumn{1}{l|}{1.765}  & \multicolumn{1}{l|}{0.784} & \multicolumn{1}{l|}{9.106}  & \multicolumn{1}{l|}{4.125}   & \multicolumn{1}{l|}{10.429}  & \multicolumn{1}{l|}{1.294}     & \multicolumn{1}{l|}{2.064}   & \multicolumn{1}{l|}{0.875}  & \multicolumn{1}{l|}{11.421}      & \multicolumn{1}{l|}{5.335}   & \multicolumn{1}{l|}{13.913}   & \multicolumn{1}{l|}{1.541}         & \multicolumn{1}{l|}{2.284}    &  0.943   \\ \hline


MQRNN & \multicolumn{1}{l|}{7.882}                & \multicolumn{1}{l|}{3.468}                & \multicolumn{1}{l|}{8.340}                & \multicolumn{1}{l|}{1.192}                & \multicolumn{1}{l|}{1.813}                & \multicolumn{1}{l|}{0.836}                & \multicolumn{1}{l|}{9.854}                & \multicolumn{1}{l|}{4.306}                & \multicolumn{1}{l|}{10.623}                & \multicolumn{1}{l|}{1.346}                & \multicolumn{1}{l|}{2.123}               & \multicolumn{1}{l|}{0.913}                & \multicolumn{1}{l|}{11.930}                & \multicolumn{1}{l|}{5.428}                & \multicolumn{1}{l|}{13.884}                & \multicolumn{1}{l|}{1.645}                & \multicolumn{1}{l|}{2.469}                & 1.165                           \\ \hline


STGCN & \multicolumn{1}{l|}{6.042}                & \multicolumn{1}{l|}{3.132}                & \multicolumn{1}{l|}{8.665}                & \multicolumn{1}{l|}{0.930}                & \multicolumn{1}{l|}{1.566}                & \multicolumn{1}{l|}{0.607}                & \multicolumn{1}{l|}{7.246}                & \multicolumn{1}{l|}{3.622}                & \multicolumn{1}{l|}{10.638}                & \multicolumn{1}{l|}{1.113}                & \multicolumn{1}{l|}{1.811}               & \multicolumn{1}{l|}{0.669}                & \multicolumn{1}{l|}{8.435}                & \multicolumn{1}{l|}{4.171}                & \multicolumn{1}{l|}{12.873}                & \multicolumn{1}{l|}{1.367}                & \multicolumn{1}{l|}{2.086}                & 0.736                             \\ \hline




STGCN+QSTCL  & \multicolumn{1}{l|}{{\ul \textbf{5.806}}}                & \multicolumn{1}{l|}{{\ul \textbf{3.027}}}                & \multicolumn{1}{l|}{{\ul \textbf{8.249}}}                & \multicolumn{1}{l|}{{\ul \textbf{0.878}}}                & \multicolumn{1}{l|}{{\ul \textbf{1.514}}}               & \multicolumn{1}{l|}{{\ul \textbf{0.586}}}                & \multicolumn{1}{l|}{{\ul \textbf{ 6.919}}}                & \multicolumn{1}{l|}{{\ul \textbf{3.488}}}                & \multicolumn{1}{l|}{{\ul \textbf{10.086}}}                & \multicolumn{1}{l|}{{\ul \textbf{1.045}}}                & \multicolumn{1}{l|}{{\ul \textbf{1.744}}}               & \multicolumn{1}{l|}{{\ul \textbf{0.648}}}                & \multicolumn{1}{l|}{{\ul \textbf{7.974}}}                & \multicolumn{1}{l|}{{\ul \textbf{3.999}}}                & \multicolumn{1}{l|}{{\ul \textbf{12.095}}}                & \multicolumn{1}{l|}{{\ul \textbf{1.257}}}                & \multicolumn{1}{l|}{{\ul \textbf{2.000}}}                &    \multicolumn{1}{l|}{{\ul \textbf{0.720}}}                              \\ \hline



DCRNN & \multicolumn{1}{l|}{5.370}                & \multicolumn{1}{l|}{2.825}                & \multicolumn{1}{l|}{7.356}                & \multicolumn{1}{l|}{0.812}                & \multicolumn{1}{l|}{1.413}                & \multicolumn{1}{l|}{0.571}                & \multicolumn{1}{l|}{6.415}                & \multicolumn{1}{l|}{3.232 }                & \multicolumn{1}{l|}{8.869}                & \multicolumn{1}{l|}{0.951}                & \multicolumn{1}{l|}{1.616}               & \multicolumn{1}{l|}{0.634}                & \multicolumn{1}{l|}{7.578 }                & \multicolumn{1}{l|}{3.760}                & \multicolumn{1}{l|}{10.828 }                & \multicolumn{1}{l|}{1.133}                & \multicolumn{1}{l|}{1.880 }                & 0.715                           \\ \hline


1DCRNN+QSTCL   & \multicolumn{1}{l|}{{\ul \textbf{5.167}}}                & \multicolumn{1}{l|}{{\ul \textbf{2.684}}}                & \multicolumn{1}{l|}{{\ul \textbf{7.231}}}                & \multicolumn{1}{l|}{{\ul \textbf{0.783}}}                & \multicolumn{1}{l|}{{\ul \textbf{1.364}}}               & \multicolumn{1}{l|}{{\ul \textbf{0.506}}}                & \multicolumn{1}{l|}{{\ul \textbf{6.304}}}                & \multicolumn{1}{l|}{{\ul \textbf{3.169}}}                & \multicolumn{1}{l|}{{\ul \textbf{8.795}}}                & \multicolumn{1}{l|}{{\ul \textbf{0.894}}}                & \multicolumn{1}{l|}{{\ul \textbf{1.514}}}               & \multicolumn{1}{l|}{{\ul \textbf{0.576}}}                & \multicolumn{1}{l|}{{\ul \textbf{7.495}}}                & \multicolumn{1}{l|}{{\ul \textbf{3.684}}}                & \multicolumn{1}{l|}{{\ul \textbf{12.573}}}                & \multicolumn{1}{l|}{{\ul \textbf{1.053}}}                & \multicolumn{1}{l|}{{\ul \textbf{1.801}}}                &    \multicolumn{1}{l|}{{\ul \textbf{0.649}}}                              \\ \hline


GWN & \multicolumn{1}{l|}{5.420}                & \multicolumn{1}{l|}{2.805}                & \multicolumn{1}{l|}{7.332}                & \multicolumn{1}{l|}{0.803}                & \multicolumn{1}{l|}{1.402}                & \multicolumn{1}{l|}{0.562}                & \multicolumn{1}{l|}{6.398}                & \multicolumn{1}{l|}{3.185}                & \multicolumn{1}{l|}{8.771}                & \multicolumn{1}{l|}{0.929}                & \multicolumn{1}{l|}{1.593}               & \multicolumn{1}{l|}{.621}                & \multicolumn{1}{l|}{7.42}                & \multicolumn{1}{l|}{3.637}                & \multicolumn{1}{l|}{10.449}                & \multicolumn{1}{l|}{1.081}                & \multicolumn{1}{l|}{1.818}                & 0.691                           \\ \hline


GWN+QSTCL  & \multicolumn{1}{l|}{{\ul \textbf{5.281}}}                & \multicolumn{1}{l|}{{\ul \textbf{2.740}}}                & \multicolumn{1}{l|}{{\ul \textbf{7.149}}}                & \multicolumn{1}{l|}{{\ul \textbf{0.781}}}                & \multicolumn{1}{l|}{{\ul \textbf{1.370}}}               & \multicolumn{1}{l|}{{\ul \textbf{0.544 }}}                & \multicolumn{1}{l|}{{\ul \textbf{6.187 }}}                & \multicolumn{1}{l|}{{\ul \textbf{3.096}}}                & \multicolumn{1}{l|}{{\ul \textbf{ 8.519}}}                & \multicolumn{1}{l|}{{\ul \textbf{0.899}}}                & \multicolumn{1}{l|}{{\ul \textbf{1.548}}}               & \multicolumn{1}{l|}{{\ul \textbf{ 0.598}}}                & \multicolumn{1}{l|}{{\ul \textbf{7.144 }}}                & \multicolumn{1}{l|}{{\ul \textbf{3.510}}}                & \multicolumn{1}{l|}{{\ul \textbf{10.023}}}                & \multicolumn{1}{l|}{{\ul \textbf{1.038}}}                & \multicolumn{1}{l|}{{\ul \textbf{1.755}}}                &    \multicolumn{1}{l|}{{\ul \textbf{0.666}}}                              \\ \hline

STNorm & \multicolumn{1}{l|}{5.475}                & \multicolumn{1}{l|}{2.826}                & \multicolumn{1}{l|}{7.359}                & \multicolumn{1}{l|}{0.808}                & \multicolumn{1}{l|}{1.413}                & \multicolumn{1}{l|}{0.561}                & \multicolumn{1}{l|}{6.434}                & \multicolumn{1}{l|}{3.192}                & \multicolumn{1}{l|}{8.799}                & \multicolumn{1}{l|}{0.934}                & \multicolumn{1}{l|}{1.596}               & \multicolumn{1}{l|}{0.614}                & \multicolumn{1}{l|}{7.443}                & \multicolumn{1}{l|}{3.627}                & \multicolumn{1}{l|}{10.500}                & \multicolumn{1}{l|}{1.085}                & \multicolumn{1}{l|}{1.814}                &         0.683                  \\ \hline


STNorm-QSTCL & \multicolumn{1}{l|}{{\ul \textbf{5.376}}}                & \multicolumn{1}{l|}{{\ul \textbf{2.773} }}               & \multicolumn{1}{l|}{{\ul \textbf{7.278}  }}              & \multicolumn{1}{l|}{{\ul \textbf{0.796}}}                & \multicolumn{1}{l|}{{\ul \textbf{1.387}   }}             & \multicolumn{1}{l|}{{\ul \textbf{ 0.550}}}                & \multicolumn{1}{l|}{{\ul \textbf{6.296}}}                & \multicolumn{1}{l|}{{\ul \textbf{3.134}  }}              & \multicolumn{1}{l|}{{\ul \textbf{ 8.688 } }}               & \multicolumn{1}{l|}{{\ul \textbf{0.920}}}                & \multicolumn{1}{l|}{{\ul \textbf{1.567}}}              & \multicolumn{1}{l|}{{\ul \textbf{ 0.601}}}                & \multicolumn{1}{l|}{{\ul \textbf{7.278}}}                & \multicolumn{1}{l|}{{\ul \textbf{3.566}}}                & \multicolumn{1}{l|}{{\ul \textbf{10.392}}}                & \multicolumn{1}{l|}{{\ul \textbf{1.069}}}                & \multicolumn{1}{l|}{{\ul \textbf{1.783}}}                &          {\ul \textbf{0.670}}                \\ \hline

SCINet & \multicolumn{1}{l|}{5.902}                & \multicolumn{1}{l|}{3.278}                & \multicolumn{1}{l|}{8.940}                & \multicolumn{1}{l|}{0.977}                & \multicolumn{1}{l|}{1.639}                & \multicolumn{1}{l|}{0.708}                & \multicolumn{1}{l|}{6.713}                & \multicolumn{1}{l|}{3.671}                & \multicolumn{1}{l|}{10.374}                & \multicolumn{1}{l|}{1.112}                & \multicolumn{1}{l|}{1.836}               & \multicolumn{1}{l|}{0.761}                & \multicolumn{1}{l|}{7.794}                & \multicolumn{1}{l|}{4.221}                & \multicolumn{1}{l|}{12.305}                & \multicolumn{1}{l|}{1.312}                & \multicolumn{1}{l|}{2.111}                &           0.872                \\ \hline

SCINet-QSTCL & \multicolumn{1}{l|}{{\ul \textbf{5.814}}}                & \multicolumn{1}{l|}{{\ul \textbf{3.216}}}                & \multicolumn{1}{l|}{{\ul \textbf{8.664}}}                & \multicolumn{1}{l|}{{\ul \textbf{0.967}}}                & \multicolumn{1}{l|}{{\ul \textbf{1.608}}}                & \multicolumn{1}{l|}{{\ul \textbf{40.679}}}                & \multicolumn{1}{l|}{{\ul \textbf{6.637} }}               & \multicolumn{1}{l|}{{\ul \textbf{3.609}  }}              & \multicolumn{1}{l|}{{\ul \textbf{10.154}}}                & \multicolumn{1}{l|}{{\ul \textbf{1.097}}}                & \multicolumn{1}{l|}{{\ul \textbf{1.804}}}               & \multicolumn{1}{l|}{{\ul \textbf{0.728}}}              & \multicolumn{1}{l|}{{\ul \textbf{7.687}}}                & \multicolumn{1}{l|}{{\ul \textbf{4.147}}}                & \multicolumn{1}{l|}{{\ul \textbf{12.042}}}                & \multicolumn{1}{l|}{{\ul \textbf{1.285}}}                & \multicolumn{1}{l|}{{\ul \textbf{2.073}}}                &          {\ul \textbf{ 0.823}}                \\ \hline



STAEFormer & \multicolumn{1}{l|}{5.214}                & \multicolumn{1}{l|}{2.707}                & \multicolumn{1}{l|}{7.018}                & \multicolumn{1}{l|}{0.765}                & \multicolumn{1}{l|}{1.353}                & \multicolumn{1}{l|}{0.538}                & \multicolumn{1}{l|}{6.158}                & \multicolumn{1}{l|}{3.042}                & \multicolumn{1}{l|}{8.353}                & \multicolumn{1}{l|}{0.886 }                & \multicolumn{1}{l|}{1.521}               & \multicolumn{1}{l|}{0.588}                & \multicolumn{1}{l|}{7.153}                & \multicolumn{1}{l|}{13.43}                & \multicolumn{1}{l|}{10.047}                & \multicolumn{1}{l|}{1.036}                & \multicolumn{1}{l|}{1.717}                &       0.647                 \\ \hline

% | 3  Horizon | RMSE:  29.292; MAE:  17.589; MAPE: 11.993; Q10: 4.190; Q50: 8.794; Q90: 3.921;
% | 6  Horizon | RMSE:  30.931; MAE:  18.371; MAPE: 12.435; Q10: 4.486; Q50: 9.186; Q90: 4.141;
% | 12 Horizon | RMSE:  32.922; MAE:  19.543; MAPE: 13.171; Q10: 4.844; Q50: 9.772; Q90: 4.482;


STAEFormer-QSTCL & \multicolumn{1}{l|}{{\ul \textbf{5.038}}}                & \multicolumn{1}{l|}{{\ul \textbf{2.629}}}                & \multicolumn{1}{l|}{{\ul \textbf{6.789}}}               & \multicolumn{1}{l|}{{\ul \textbf{0.743}}}                & \multicolumn{1}{l|}{{\ul \textbf{1.315}}}                & \multicolumn{1}{l|}{{\ul \textbf{0.524}}}                & \multicolumn{1}{l|}{{\ul \textbf{5.948}}}                & \multicolumn{1}{l|}{{\ul \textbf{2.956}}}                & \multicolumn{1}{l|}{{\ul \textbf{8.100}}}                & \multicolumn{1}{l|}{{\ul \textbf{0.864}}}                & \multicolumn{1}{l|}{{\ul \textbf{1.478}}}               & \multicolumn{1}{l|}{{\ul \textbf{0.575}}}                & \multicolumn{1}{l|}{{\ul \textbf{6.941}}}                & \multicolumn{1}{l|}{{\ul \textbf{3.349}}}                & \multicolumn{1}{l|}{{\ul \textbf{9.703}}}                & \multicolumn{1}{l|}{{\ul \textbf{1.010}}}                & \multicolumn{1}{l|}{{\ul \textbf{1.675}}}                &          {\ul \textbf{0.637}}                 \\ \hline


\end{tabular}
\end{table*}
